Mitigating Context-Memory Conflicts in LLMs through Dynamic Cognitive Reconciliation Decoding

Large language models accumulate extensive parametric knowledge through pre-training. However, knowledge conflicts occur when outdated or incorrect parametric knowledge conflicts with external knowledge in the context. Existing methods address knowledge conflicts through contrastive decoding, but in conflict-free scenarios, static approaches disrupt output distribution. Other dynamic decoding methods attempt to measure the degree of conflict but still struggle with complex real-world situations. In this paper, we propose a two-stage decoding method called Dynamic Cognitive Reconciliation Decoding (DCRD), to predict and mitigate context-memory conflicts. DCRD first analyzes the attention map to assess context fidelity and predict potential conflicts. Based on this prediction, the input is directed to one of two decoding paths: (1) greedy decoding, or (2) context fidelity-based dynamic decoding. This design enables DCRD to handle conflicts efficiently while maintaining high accuracy and decoding efficiency in conflict-free cases. Additionally, to simulate scenarios with frequent knowledge updates, we constructed ConflictKG, a knowledge conflict QA benchmark. Experiments on four LLMs across six QA datasets show that DCRD outperforms all baselines, achieving state-of-the-art performance.

==> table/main.tex <==

\begin{table*}[t]
\small
\renewcommand{\arraystretch}{1.30}
\belowrulesep=0pt
\aboverulesep=0pt
\centering
\resizebox{\linewidth}{!}{
    \begin{tabular}{c|c|ccccc|c}
    \toprule
    \rowcolor[gray]{0.9}
    
     & & 
    \multicolumn{2}{c}{\textbf{General QA}} & 
    \multicolumn{2}{c}{\textbf{Knowledge Conflict QA}} & 
    \multicolumn{1}{c|}{\textbf{Our Benchmark}}  & 
    \\ 
    %\cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-7}
    \rowcolor[gray]{0.9}
   \multirow{-2}{*}{\textbf{Model}} &  \multirow{-2}{*}{\textbf{Decoding}} & 
    \phantom{0} \textbf{NQ} \phantom{0} & \textbf{SQUAD} & 
    \textbf{NQ-Swap} & \textbf{Counterfacts} & 
    \textbf{ConflictKG} &  \multirow{-2}{*}{ \phantom{0} \textbf{Avg.} \phantom{0}}
    \\ 
    \midrule
    \multirow{5}{*}{Llama2-7B} 
     & \cellcolor[gray]{0.945}Greedy & \cellcolor[gray]{0.945}51.9 &  \cellcolor[gray]{0.945}71.6 & \cellcolor[gray]{0.945}36.5 & \cellcolor[gray]{0.945}33.8 & \cellcolor[gray]{0.945}66.0  & \cellcolor[gray]{0.945}52.0\\
    \cmidrule(){2-8}
     & CAD & 50.3$_{\mathclap{\hspace{1.2em}\small\darkred{\textbf{-1.6}}}}$ & 67.7$_{\mathclap{\hspace{1.2em}\small\darkred{\textbf{-3.9}}}}$ & 47.5$_{\mathclap{\hspace{1.2em}\small\darkgreen{\textbf{11.0}}}}$ & 47.4$_{\mathclap{\hspace{1.2em}\small\darkgreen{\textbf{13.6}}}}$ & 77.5$_{\mathclap{\hspace{1.2em}\small\darkgreen{\textbf{11.5}}}}$ & 58.1$_{\mathclap{\hspace{0.9em}\small\darkgreen{\textbf{6.1}}}}$ \\
     & COIECD & 59.9$_{\mathclap{\hspace{0.9em}\small\darkgreen{\textbf{8.0}}}}$ & 76.0$_{\mathclap{\hspace{0.9em}\small\darkgreen{\textbf{4.4}}}}$ & 48.9$_{\mathclap{\hspace{1.2em}\small\darkgreen{\textbf{12.4}}}}$ & 48.4$_{\mathclap{\hspace{1.2em}\small\darkgreen{\textbf{14.6}}}}$ &75.9$_{\mathclap{\hspace{0.9em}\small\darkgreen{\textbf{9.9}}}}$  & 61.8$_{\mathclap{\hspace{0.9em}\small\darkgreen{\textbf{9.8}}}}$ \\
     & ADACAD & 65.4$_{\mathclap{\hspace{1.2em}\small\darkgreen{\textbf{13.5}}}}$ & 74.6$_{\mathclap{\hspace{0.9em}\small\darkgreen{\textbf{3.0}}}}$ & 46.1$_{\mathclap{\hspace{0.9em}\small\darkgreen{\textbf{9.6}}}}$ & 44.3$_{\mathclap{\hspace{1.2em}\small\darkgreen{\textbf{10.5}}}}$ & 72.0$_{\mathclap{\hspace{0.9em}\small\darkgreen{\textbf{6.0}}}}$ & 60.5$_{\mathclap{\hspace{0.9em}\small\darkgreen{\textbf{8.5}}}}$ \\
    \cmidrule(){2-8}
     & \cellcolor[HTML]{FDF5F1}\textbf{\ourapproach (Ours)} & \cellcolor[HTML]{FDF5F1} \textbf{68.4}$_{\mathclap{\hspace{1.2em}\small\darkgreen{\textbf{16.5}}}}$ & \cellcolor[HTML]{FDF5F1}\textbf{83.2}$_{\mathclap{\hspace{1.2em}\small\darkgreen{\textbf{11.6}}}}$& \cellcolor[HTML]{FDF5F1}\textbf{54.2}$_{\mathclap{\hspace{1.2em}\small\darkgreen{\textbf{17.7}}}}$ & \cellcolor[HTML]{FDF5F1}\textbf{57.4}$_{\mathclap{\hspace{1.2em}\small\darkgreen{\textbf{23.6}}}}$& \cellcolor[HTML]{FDF5F1}\textbf{81.1}$_{\mathclap{\hspace{1.2em}\small\darkgreen{\textbf{15.1}}}}$ & \cellcolor[HTML]{FDF5F1}\textbf{68.9}$_{\mathclap{\hspace{1.2em}\small\darkgreen{\textbf{16.9}}}}$ \\
    \midrule
    \midrule
    \multirow{5}{*}{Llama2-13B} 
     & \cellcolor[gray]{0.945}Greedy & \cellcolor[gray]{0.945}64.3 & \cellcolor[gray]{0.945}73.9 & \cellcolor[gray]{0.945}36.4 & \cellcolor[gray]{0.945}53.0 & \cellcolor[gray]{0.945}73.7 & \cellcolor[gray]{0.945}60.3 \\
    \cmidrule(){2-8}
     & CAD & 51.3$_{\mathclap{\hspace{1.5em}\small\darkred{\textbf{-13.0}}}}$ & 72.7$_{\mathclap{\hspace{0.9em}\small\darkred{\textbf{-1.2}}}}$ & 53.9$_{\mathclap{\hspace{1.2em}\small\darkgreen{\textbf{17.5}}}}$ & 62.3$_{\mathclap{\hspace{0.9em}\small\darkgreen{\textbf{9.3}}}}$ & 80.1$_{\mathclap{\hspace{0.9em}\small\darkgreen{\textbf{6.4}}}}$ & 64.1$_{\mathclap{\hspace{0.9em}\small\darkgreen{\textbf{3.8}}}}$ \\
     & COIECD & 68.6$_{\mathclap{\hspace{0.9em}\small\darkgreen{\textbf{4.3}}}}$ & 78.9$_{\mathclap{\hspace{0.9em}\small\darkgreen{\textbf{5.0}}}}$ & 54.0$_{\mathclap{\hspace{1.2em}\small\darkgreen{\textbf{17.6}}}}$ & 56.8$_{\mathclap{\hspace{0.9em}\small\darkgreen{\textbf{3.8}}}}$ & 76.8$_{\mathclap{\hspace{0.9em}\small\darkgreen{\textbf{3.1}}}}$ & 67.0$_{\mathclap{\hspace{0.9em}\small\darkgreen{\textbf{6.7}}}}$  \\
     & ADACAD & 68.2$_{\mathclap{\hspace{0.9em}\small\darkgreen{\textbf{3.9}}}}$ & 76.5$_{\mathclap{\hspace{0.9em}\small\darkgreen{\textbf{2.6}}}}$ & 62.6$_{\mathclap{\hspace{1.2em}\small\darkgreen{\textbf{26.2}}}}$ & 62.5$_{\mathclap{\hspace{0.9em}\small\darkgreen{\textbf{9.5}}}}$ & 77.4$_{\mathclap{\hspace{0.9em}\small\darkgreen{\textbf{3.7}}}}$ & 69.4$_{\mathclap{\hspace{0.9em}\small\darkgreen{\textbf{9.1}}}}$ \\
    \cmidrule(){2-8}
     & \cellcolor[HTML]{FDF5F1}\textbf{\ourapproach (Ours)} & \cellcolor[HTML]{FDF5F1}\textbf{71.4}$_{\mathclap{\hspace{0.9em}\small\darkgreen{\textbf{7.1}}}}$ & \cellcolor[HTML]{FDF5F1}\textbf{79.5}$_{\mathclap{\hspace{1.2em}\small\darkgreen{\textbf{5.6}}}}$& \cellcolor[HTML]{FDF5F1}\textbf{65.5}$_{\mathclap{\hspace{1.2em}\small\darkgreen{\textbf{29.1}}}}$ &\cellcolor[HTML]{FDF5F1}\textbf{65.2}$_{\mathclap{\hspace{1.2em}\small\darkgreen{\textbf{12.2}}}}$  & \cellcolor[HTML]{FDF5F1}\textbf{86.0}$_{\mathclap{\hspace{1.2em}\small\darkgreen{\textbf{12.3}}}}$ & \cellcolor[HTML]{FDF5F1}\textbf{73.5}$_{\mathclap{\hspace{1.2em}\small\darkgreen{\textbf{13.2}}}}$ \\
    \midrule
    \midrule
    \multirow{5}{*}{Llama3-8B} 
     & \cellcolor[gray]{0.945}Greedy & \cellcolor[gray]{0.945}67.4 & \cellcolor[gray]{0.945}87.2& \cellcolor[gray]{0.945}47.2 & \cellcolor[gray]{0.945}48.1& \cellcolor[gray]{0.945}67.9 &  \cellcolor[gray]{0.945}63.6\\
    \cmidrule(){2-8}
     & CAD & 51.0$_{\mathclap{\hspace{1.5em}\small\darkred{\textbf{-16.4}}}}$ & 72.6$_{\mathclap{\hspace{1.5em}\small\darkred{\textbf{-14.6}}}}$ & 56.0$_{\mathclap{\hspace{0.9em}\small\darkgreen{\textbf{8.8}}}}$ & 57.6$_{\mathclap{\hspace{0.9em}\small\darkgreen{\textbf{9.5}}}}$ & 68.4$_{\mathclap{\hspace{1.2em}\small\darkred{\textbf{-4.7}}}}$ & 61.1$_{\mathclap{\hspace{1.2em}\small\darkred{\textbf{-2.5}}}}$ \\
     & COIECD & 68.4$_{\mathclap{\hspace{0.9em}\small\darkgreen{\textbf{1.0}}}}$ & 86.9$_{\mathclap{\hspace{1.2em}\small\darkred{\textbf{-0.3}}}}$ & 52.1$_{\mathclap{\hspace{0.9em}\small\darkgreen{\textbf{4.9}}}}$ & 52.1$_{\mathclap{\hspace{0.9em}\small\darkgreen{\textbf{4.0}}}}$ & 70.3$_{\mathclap{\hspace{0.9em}\small\darkgreen{\textbf{2.4}}}}$ & 66.0$_{\mathclap{\hspace{0.9em}\small\darkgreen{\textbf{2.4}}}}$ \\
     & ADACAD & 65.2$_{\mathclap{\hspace{1.2em}\small\darkred{\textbf{-2.2}}}}$ & 87.1$_{\mathclap{\hspace{1.2em}\small\darkred{\textbf{-0.1}}}}$ & 58.3$_{\mathclap{\hspace{1.2em}\small\darkgreen{\textbf{11.1}}}}$ & 59.0$_{\mathclap{\hspace{1.2em}\small\darkgreen{\textbf{10.9}}}}$ & 77.5$_{\mathclap{\hspace{0.9em}\small\darkgreen{\textbf{9.S6}}}}$ & 69.4$_{\mathclap{\hspace{0.9em}\small\darkgreen{\textbf{5.8}}}}$ \\
    \cmidrule(){2-8}
     & \cellcolor[HTML]{FDF5F1}\textbf{\ourapproach (Ours)} & \cellcolor[HTML]{FDF5F1}\textbf{73.4}$_{\mathclap{\hspace{0.9em}\small\darkgreen{\textbf{6.0}}}}$ &  \cellcolor[HTML]{FDF5F1}\textbf{88.9}$_{\mathclap{\hspace{0.9em}\small\darkgreen{\textbf{1.7}}}}$& \cellcolor[HTML]{FDF5F1}\textbf{65.3}$_{\mathclap{\hspace{1.2em}\small\darkgreen{\textbf{18.1}}}}$ & \cellcolor[HTML]{FDF5F1}\textbf{67.3}$_{\mathclap{\hspace{1.2em}\small\darkgreen{\textbf{19.2}}}}$  & \cellcolor[HTML]{FDF5F1}\textbf{79.5}$_{\mathclap{\hspace{1.2em}\small\darkgreen{\textbf{11.6}}}}$ & \cellcolor[HTML]{FDF5F1}\textbf{74.9}$_{\mathclap{\hspace{1.2em}\small\darkgreen{\textbf{11.3}}}}$ \\
    \midrule
    \midrule
    \multirow{5}{*}{Mistral-7B} 
     & \cellcolor[gray]{0.945}Greedy & \cellcolor[gray]{0.945}58.8 & \cellcolor[gray]{0.945}67.5& \cellcolor[gray]{0.945}45.6 & \cellcolor[gray]{0.945}41.6& \cellcolor[gray]{0.945}66.2 & \cellcolor[gray]{0.945}55.9 \\
    \cmidrule(){2-8}
     & CAD & 52.6$_{\mathclap{\hspace{1.2em}\small\darkred{\textbf{-6.2}}}}$ & 25.2$_{\mathclap{\hspace{1.5em}\small\darkred{\textbf{-42.3}}}}$ & 48.1$_{\mathclap{\hspace{0.9em}\small\darkgreen{\textbf{2.5}}}}$ & 45.8$_{\mathclap{\hspace{0.9em}\small\darkgreen{\textbf{4.2}}}}$ & 36.3$_{\mathclap{\hspace{1.5em}\small\darkred{\textbf{-29.9}}}}$ & 41.6$_{\mathclap{\hspace{1.5em}\small\darkred{\textbf{-14.3}}}}$ \\
     & COIECD & 59.1$_{\mathclap{\hspace{0.9em}\small\darkgreen{\textbf{0.3}}}}$ & 48.1$_{\mathclap{\hspace{1.2em}\small\darkred{\textbf{-19.4}}}}$ & 56.0$_{\mathclap{\hspace{1.2em}\small\darkgreen{\textbf{10.4}}}}$ & 54.0$_{\mathclap{\hspace{1.2em}\small\darkgreen{\textbf{12.4}}}}$ & 69.1$_{\mathclap{\hspace{0.9em}\small\darkgreen{\textbf{2.9}}}}$ & 57.3$_{\mathclap{\hspace{0.9em}\small\darkgreen{\textbf{1.4}}}}$ \\
     & ADACAD & 58.1$_{\mathclap{\hspace{1.2em}\small\darkred{\textbf{-0.7}}}}$ & \textbf{75.2}$_{\mathclap{\hspace{0.9em}\small\darkgreen{\textbf{7.7}}}}$ & 51.7$_{\mathclap{\hspace{0.9em}\small\darkgreen{\textbf{6.1}}}}$ & 49.8$_{\mathclap{\hspace{0.9em}\small\darkgreen{\textbf{8.2}}}}$ & 67.4$_{\mathclap{\hspace{0.9em}\small\darkgreen{\textbf{1.2}}}}$ & 60.4$_{\mathclap{\hspace{0.9em}\small\darkgreen{\textbf{4.5}}}}$ \\
    \cmidrule(){2-8}
     & \cellcolor[HTML]{FDF5F1}\textbf{\ourapproach (Ours)} & \cellcolor[HTML]{FDF5F1}\textbf{60.9}$_{\mathclap{\hspace{0.9em}\small\darkgreen{\textbf{2.1}}}}$ & \cellcolor[HTML]{FDF5F1}69.1$_{\mathclap{\hspace{0.9em}\small\darkgreen{\textbf{1.6}}}}$  & \cellcolor[HTML]{FDF5F1}\textbf{58.3}$_{\mathclap{\hspace{1.2em}\small\darkgreen{\textbf{12.7}}}}$ &\cellcolor[HTML]{FDF5F1}\textbf{57.9}$_{\mathclap{\hspace{1.2em}\small\darkgreen{\textbf{16.3}}}}$  & \cellcolor[HTML]{FDF5F1}\textbf{72.6}$_{\mathclap{\hspace{0.9em}\small\darkgreen{\textbf{6.4}}}}$ &  \cellcolor[HTML]{FDF5F1}\textbf{63.8}$_{\mathclap{\hspace{0.9em}\small\darkgreen{\textbf{7.9}}}}$\\
    \bottomrule
    \end{tabular}
}
\caption{Conflict mitigation performance on general QA datasets, knowledge conflict QA datasets, and ConflictQA. DCRD outperforms all baselines. Greedy represents greedy decoding. The number in the subscript indicates the difference in greedy decoding compared to the baseline.\textcolor{blue}{The black numerical values denote the accuracy of the methods on each benchmark. The subscripts represent the performance difference between the current method and the baseline, where red indicates performance degradation and green indicates performance improvement.}}
\label{tab:main_qa}
\end{table*}

==> table/prompt2.tex <==
\begin{table*}[t]
\caption {Prompt for conflict context generation}
\resizebox{\linewidth}{!}{
    \centering
    \renewcommand{\arraystretch}{1.0}
\begin{tabular}{l}
\toprule
\textbf{Prompt for conflict context generation}       
                 \\ 
\hline
\addlinespace[6pt]
\begin{tabular}[c]{@{}l@{}}
\parbox[c]{15.6cm}{

You are a knowledge conflict context generation expert. You will be provided with a question, reference context, and the correct answer based on that context. Your task is to fabricate a new answer that contradicts the correct answer (i.e., the facts) and create a new conflicting context based on this new answer, so that other models can answer the question using the new context and provide the new answer.\\ \\
1. Fabricate a new answer that is different from the original answer, ensuring that the new answer has a similar structure and type to the original.\\
2. Based on the original context and the fabricated new answer, generate a new conflict context. The parts of the new context corresponding to the original answer should conflict with the original context, reflecting the incorrect answer.\\
3. The generated new context should maintain fluency and coherence.\\
4. The final generation format should be: \#\#conflict answer: a new answer \#\#. \#\#conflict context: a new context\#\#.\\ 

Here is the reference information:\\ 
Question: <QUESTION> \\
Topic Entity: <ENTITY> \\
Original Answer: <ANSWER> \\
Original Context: <CONTEXT>\\ \\
Please generate a new answer (that contradicts the original answer) and a new conflicting context (that contradicts the original context):
    }
\end{tabular} \\
\addlinespace[4pt]
\bottomrule
\end{tabular}}
    
    % \vspace{-0.5em}
    \label{tab:prompt2}
\end{table*}

==> table/prompt3.tex <==
\begin{table*}[t]
\caption {Prompt for noisy context generation}
\resizebox{\linewidth}{!}{
    \centering
    \renewcommand{\arraystretch}{1.20}
\begin{tabular}{l}
\toprule
\textbf{Prompt for noisy context generation}       
                 \\ 
\hline
\addlinespace[6pt]
\begin{tabular}[c]{@{}l@{}}
\parbox[c]{15.6cm}{
You are an expert in generating noisy contexts. You will be given a question, a reference context, and the correct answer based on that context. Your task is to generate a noisy context that simulates the situation in a retrieval system where the system might return content that is irrelevant to the question or context.\\

Task Requirements:\\
1. Based on the given information, generate a noisy context. The noisy context should be completely unrelated to the original context, but it should still be fluent and appropriate in language.\\
2. The content of the noisy context must not affect the correctness of the original context. In other words, despite the addition of the noisy context, the original answer should still be accurate based on the new context.\\
3. The noisy context should not contain any misleading or incorrect answers. It should simply be content that is unrelated to the original question and context.\\
4. The final format should be: \#\#Noisy context: output \#\#.\\ 

Here is the reference information: \quad Question: <QUESTION> \quad Entity: <ENTITY> \quad Answer: <ANSWER> \quad Original Context: <CONTEXT>\\ \\
Please generate a noisy context:
    }
\end{tabular} \\
\addlinespace[4pt]
\bottomrule
\end{tabular}}
    
    % \vspace{-0.5em}
    \label{tab:prompt3}
\end{table*}
